GIMO: Gaze-Informed Human Motion Prediction in Context

Predicting human motion is critical for assistive robots and AR/VR applications, where the interaction with humans needs to be safe and comfortable. Meanwhile, an accurate prediction depends on understanding both the scene context and human intentions. Even though many works study scene-aware human motion prediction, the latter is largely underexplored due to the lack of ego-centric views that disclose human intent and the limited diversity in motion and scenes. To reduce the gap, we propose a large-scale human motion dataset that delivers high-quality body pose sequences, scene scans, as well as ego-centric views with the eye gaze that serves as a surrogate for inferring human intent. By employing inertial sensors for motion capture, our data collection is not tied to specific scenes, which further boosts the motion dynamics observed from our subjects. We perform an extensive study of the benefits of leveraging the eye gaze for ego-centric human motion prediction with various state-of-the-art architectures. Moreover, to realize the full potential of the gaze, we propose a novel network architecture that enables bidirectional communication between the gaze and motion branches. Our network achieves the top performance in human motion prediction on the proposed dataset, thanks to the intent information from eye gaze and the denoised gaze feature modulated by the motion. Code and data can be found at https://github.com/y-zheng18/GIMO.

==> figs_tables/fig_cross.tex <==
\begin{figure}[t!]
    \centering
    \includegraphics[width=\linewidth]{figures/crossmodal_transformer.pdf}
    \caption{The architecture of crossmodal transformer~\cite{jaegle2021perceiver}. \yanchao{we should combine this figure with Fig.4, either insert it into Fig.4 or just get rid of it? as it is not our main contribution.} \yang{I think the figure is important. The reviewers might not know this network. otherwise we need to explain very clear in the text.}}
    \label{fig:cross}
 \end{figure}

==> figs_tables/fig_device.tex <==
\begin{figure}[t!]
    \centering
    \includegraphics[width=\linewidth]{figures/device.pdf}
    \vspace{-15pt}
    \caption{The device to collect our dataset.\yanchao{polish, e.g., the hololens image is too dark. no need to have two images in the middle? Maybe just one third view of the person with the headset and the IMUs?} \yang{changed}}
    \vspace{-10pt}
    \label{fig:device}
 \end{figure}
